Cost Function Unrolling in Unsupervised Optical Flow

Steepest descent algorithms, which are commonly used in deep learning, use the gradient as the descent direction, either as-is or after a direction shift using preconditioning. In many scenarios calculating the gradient is numerically hard due to complex or non-differentiable cost functions, specifically next to singular points. In this work we focus on the derivation of the Total Variation semi-norm commonly used in unsupervised cost functions. Specifically, we derive a differentiable proxy to the hard L1 smoothness constraint in a novel iterative scheme which we refer to as Cost Unrolling. Producing more accurate gradients during training, our method enables finer predictions of a given DNN model through improved convergence, without modifying its architecture or increasing computational complexity. We demonstrate our method in the unsupervised optical flow task. Replacing the L1 smoothness constraint with our unrolled cost during the training of a well known baseline, we report improved results on both MPI Sintel and KITTI 2015 unsupervised optical flow benchmarks. Particularly, we report EPE reduced by up to 15.82% on occluded pixels, where the smoothness constraint is dominant, enabling the detection of much sharper motion edges.

==> figures/fig_ablations_T.tex <==
\begin{figure*}
\setlength{\fboxrule}{2pt}
\setlength{\fboxsep}{2pt}
\begin{center}
%\fbox{\includegraphics[trim=90 55 70 0, width=.95\linewidth]{cvpr_unrolling.pdf}}
\includegraphics[width=1\linewidth]{figures/files/ablations_T.png}
   \caption{\textbf{Number of cost function updates.} We compare several settings for the number of update steps $T$ carried during finetuning. Images $(a),(b),(c)$ show visualizations of flows predicted by models finetuned using $T=1,2,4$ respectively. Images $(d)$ and $(e)$ are the ground truth flow and the input reference image. We find increasing the number of update steps improves the ability of our flow estimator to capture finer flow details.}
   \label{fig:ablation_T}
\end{center}
\end{figure*}

==> figures/fig_flowEst.tex <==
\begin{figure*}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\linewidth]{figures/files/FlowEst2.png}
\end{center}
    \caption{\textbf{Our DNN flow estimator unit.} 
    We adopt the ARFlow \cite{liu2020learning} framework, a recently published PWC-Net \cite{Sun2018PWC-Net} based flow architecture, as our flow estimator backbone.
    A multi-scale feature pyramid is constructed. The Warp, Correlation, Flow (W.C.F) unit is shared between all pyramid levels (shown in right image), with each level using a $1\times1$ convolution layer for dimensions alignment. At each level, the features corresponding to the target image $\mathbf{x}_2^\ell$ are warped using a coarse $\times2$ upsampled flow estimate from a higher level $\uparrow_2 \mathbf{F}^{\ell+1}$. A cost volume $\mathbf{cv}^\ell$ is generated measuring the correlation between features of the reference image $\mathbf{x}_1^\ell$ and the warped features $\mathbf{\hat{x}}_2^\ell$. The cost volume $\mathbf{cv}^\ell$, features of the reference image $\mathbf{x}_1^\ell$ and the upsampled coarse flow estimate $\uparrow_2\mathbf{F}^{\ell+1}$ are concatenated and inserted to a sub-network which outputs a finer flow estimate at each level $\mathbf{F}^\ell$.}
\label{fig:flow_est}
\end{figure*}

==> figures/fig_image_denoising.tex <==
\begin{figure*}[t]
\centering
\subfloat[]{%
\includegraphics[width=0.8\linewidth]{figures/files/denoising1.png}
\label{denoising1}
 }
 \\
\hfil
\subfloat[]{%
\includegraphics[width=0.8\linewidth]{figures/files/denoising2.png}
\label{denoising2}
}
\caption{Hyperparameter ablations.}
\label{fig_ablations}
\end{figure*}


==> figures/fig_rebuttal.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/files/denoising1.png}
         \caption{Error reduced by \textbf{12.56\%}.}
         \label{fig:denoising1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/files/denoising2.png}
         \caption{Error reduced by \textbf{19.29\%}.}
         \label{fig:denoising2}
     \end{subfigure}
        \caption{\textbf{Synthetic problem - more tested scenarios.} Presented are more generated PC signals and corresponding prediction errors.}
        \label{fig:denoising}
\end{figure*}

==> figures/fig_toy_sigs.tex <==
\begin{figure}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[trim= 0 0 10 10, width=1\linewidth]{figures/files/new_tv_sigs.png}
\end{center}
   \caption{\textbf{PC signal prediction example - target vs. predicted signals.}
   Displayed is a close up on a generated target signal, its samples and signals predicted by models trained using either standard TV regularization or our unrolled constraint. As can be seen, our unrolled cost overcomes the staircasing effect, promoting a solution which is both smooth and edge preserving.}
\label{fig:toy_sigs}
\end{figure}

==> figures/sup_ablations.tex <==
\begin{figure*}[t]
\centering
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/huber_preds.png}
\label{huber_pred}
}
\hfil
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/huber_grads.png}
\label{huber_grads}
}
\\
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/charb_preds.png}
\label{charb_preds}
}
\hfil
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/charb_grads.png}
\label{charb_grads}
}
\hfil
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/admm_preds.png}
\label{admm_preds}
}
\hfil
\subfloat[]{%
\includegraphics[width=0.4\linewidth]{figures/files/admm_grads.png}
\label{admm_grads}
}
\caption{ֿ\textbf{Signal prediction.} Hyperparameters study.}
\label{fig_ablations}
\end{figure*}


==> figures/sup_charb_grads.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/charb_grads.png}
\end{center}
   \caption{Charbonnier loss ablations - recorded gradient norms}
\label{fig:charb_grad}
\end{figure}

==> figures/sup_charb_preds.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/charb_preds.png}
\end{center}
   \caption{Charbonnier loss ablations - recorded prediction errors}
\label{fig:charb_pred}
\end{figure}

==> figures/sup_denoising_results.tex <==
\begin{figure*}
%\setlength{\fboxrule}{2pt}
%\setlength{\fboxsep}{2pt}
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/denoising_examples_supp.png}
   \caption{\textbf{Further image denoising results.}}
   \label{fig:sup_denoising}
\end{center}
\end{figure*}

==> figures/sup_flowest.tex <==
\begin{figure*}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\linewidth]{figures/files/FlowEst2.png}
\end{center}
    \caption{\textbf{Our DNN flow estimator unit.} 
    We adopt the ARFlow \cite{liu2020learning} framework, a recently published PWC-Net \cite{Sun2018PWC-Net} based flow architecture, as our flow estimator backbone.
    A multi-scale feature pyramid is constructed. The Warp, Correlation, Flow (W.C.F) unit is shared between all pyramid levels (shown in right image), with each level using a $1\times1$ convolution layer for dimensions alignment. At each level, the features corresponding to the target image $\mathbf{x}_2^\ell$ are warped using a coarse $\times2$ upsampled flow estimate from a higher level $\uparrow_2 \mathbf{F}^{\ell+1}$. A cost volume $\mathbf{cv}^\ell$ is generated measuring the correlation between features of the reference image $\mathbf{x}_1^\ell$ and the warped features $\mathbf{\hat{x}}_2^\ell$. The cost volume $\mathbf{cv}^\ell$, features of the reference image $\mathbf{x}_1^\ell$ and the upsampled coarse flow estimate $\uparrow_2\mathbf{F}^{\ell+1}$ are concatenated and inserted to a sub-network which outputs a finer flow estimate at each level $\mathbf{F}^\ell$.}
\label{fig:flow_est}
\end{figure*}

==> figures/sup_huber_grads.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/huber_grads.png}
\end{center}
   \caption{Huber loss ablations - recorded gradient norms}
\label{fig:huber_grad}
\end{figure}

==> figures/sup_huber_preds.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/huber_pred.png}
\end{center}
   \caption{Huber loss ablations - recorded prediction errors}
\label{fig:huber_pred}
\end{figure}

==> figures/sup_images.tex <==
\begin{figure*}
%\setlength{\fboxrule}{2pt}
%\setlength{\fboxsep}{2pt}
\begin{center}
\includegraphics[width=1\linewidth]{figures/files/images_data.png}
   \caption{\textbf{Image denoising data.}
   Our test data consists of 14 images commonly used for image denoising.}
   \label{fig:image_data}
\end{center}
\end{figure*}

==> figures/sup_toy_graphs.tex <==
\begin{figure*}
%\setlength{\fboxrule}{2pt}
%\setlength{\fboxsep}{2pt}
\begin{center}
%\fbox{\includegraphics[trim=90 55 70 0, width=.95\linewidth]{cvpr_unrolling.pdf}}
\includegraphics[trim=10 10 0 0, width=1\linewidth]{figures/files/sup_tv_graphs.png}
   \caption{\textbf{Synthetic problem - gradients recorded during training.} Displayed are gradients recorded during training.}
   \label{fig:sup_toy_graphs}
\end{center}
\end{figure*}

==> tables/complexity.tex <==
\begin{table}
\begin{center}
\begin{tabular}{l c c} 
    \toprule
    \textbf{Method} & \textbf{Memory} & \textbf{Runtime} \\
    \midrule
    Standard TV                 & 4.326Gi   & 51ms \\
    \textbf{Unrolled Cost (Ours)}      & \textbf{4.285Gi}   & 51ms \\
    \bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Computational complexity.} 
    Our method consumes slightly less memory during training and preserves runtime, hence 
    replacing TV regularization with our unrolled cost enables improved results with no added complexity.
%We compare several settings for the number of update steps carried at the cost function. We measure the AEPE of models pretrained on the MPI Sintel raw movie using the parameters described in section \ref{params}, and finetuned using various $T$ values. Increasing $T$ brings a performance boost, enabling our flow estimator to capture finer motion details as shown in figure \ref{fig:ablation_T}. 
}
\label{ta:comp}
\end{table}

==> tables/image_results.tex <==
\begin{table}
\begin{center}
\begin{tabular*}{.8\linewidth}{@{\extracolsep{\fill}} l | l | l | c | c  c  c}
    \toprule
    \multirow{2}{*}{\textbf{Image}} & 
    \multirow{2}{*}{$\boldsymbol{\sigma}$} & 
    \multirow{2}{*}{\textbf{Method}} & 
    \multirow{2}{*}{\textbf{PSNR [dB]}} & 
    \multicolumn{3}{c}{\textbf{pSSIM}} \\
    & & & & \emph{Red} & \emph{Cyan} & \emph{Green} \\
    \midrule
    \emph{Tower}    & 50    & DIP-TV \cite{liu2019image}    & 25.88 & 0.6533 & 0.7790 & 0.7924 \\
    \emph{Tower}    & 50    & \textbf{DIP-Unrolled (Ours)}           & \textbf{25.89} & \textbf{0.7203} & \textbf{0.7798} & \textbf{0.7983} \\
    \midrule
    \emph{Monarch}  & 75    & DIP-TV \cite{liu2019image}    & 22.56 & 0.8916 & 0.8617 & - \\
    \emph{Monarch}  & 75    & \textbf{DIP-Unrolled (Ours)}           & \textbf{22.66} & \textbf{0.9048} & \textbf{0.8758} & - \\
    \bottomrule
\end{tabular*}
\end{center}
\caption{\textbf{Image denoising quantitative results.} 
pSSIM and PSNR measured between original and reconstructed images are reported for two scenarios. The added noise level is described by $\sigma$. Our method features improved capability of restoring finer details, which is evident both numerically (pSSIM) and visually (see fig. \ref{fig:denoising}), while preserving PSNR, compared to TV regularization.
}
\label{ta:denoising_spec}
\end{table}



==> tables/image_results_spec_obs.tex <==
\begin{table}
\begin{center}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l | l | l | c  c  c}
    \toprule
    \multirow{2}{*}{\textbf{Image}} & 
    \multirow{2}{*}{$\boldsymbol{\sigma}$} & 
    \multirow{2}{*}{\textbf{Method}} & 
    \multicolumn{3}{c}{\textbf{pSSIM}} \\
    & & & \emph{Red} & \emph{Cyan} & \emph{Green} \\
    \midrule
    \multirow{2}{*}{\emph{Tower}}    & \multirow{2}{*}{50}    & DIP-TV        & 0.6533 & 0.7790 & 0.7924 \\
    &  & \textbf{Ours} & \textbf{0.7203} & \textbf{0.7798} & \textbf{0.7983} \\
    \midrule
    \multirow{2}{*}{\emph{Monarch}}  & \multirow{2}{*}{75}    & DIP-TV        & 0.8916 & 0.8617 & - \\
    &  & \textbf{Ours} & \textbf{0.9048} & \textbf{0.8758} & - \\
    \bottomrule
\end{tabular*}
\end{center}
\caption{\textbf{Example denoising results.} 
Measured pSSIM for selected patches of interest are reported for two scenarios (see fig. \ref{fig:denoising}). The added noise level is described by $\sigma$. Our method features improved capability of restoring finer details, which is evident both numerically (pSSIM) and visually.
}
\label{ta:denoising_spec}
\end{table}



==> tables/image_resutls_full.tex <==
\begin{table*}
\begin{center}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l | l | c c c c c c c}
    \toprule
    \multirow{2}{*}{\textbf{Noise Level}} & 
    \multirow{2}{*}{\textbf{Method}} & 
    \multicolumn{7}{c}{\textbf{Images}} \\
     & & \emph{1} & \emph{2} & \emph{3} & \emph{4} & \emph{5} & \emph{6} & \emph{7}  \\
    \midrule
    \multirow{2}{*}{$\sigma=25$} & DIP-TV & 
    $22.89\pm0.04$ & $26.27\pm0.51$ & $29.39\pm0.11$ & $28.10\pm0.06$ & $25.87\pm0.18$ & $28.47\pm0.04$ & $27.61\pm0.13$ \\
    & Ours &
    $22.80\pm0.17$ & $26.52\pm0.21$ & $29.32\pm0.15$ & $28.04\pm0.21$ & $26.17\pm0.08$ & $28.43\pm0.03$ & $27.56\pm0.03$ \\
    \midrule
    \multirow{2}{*}{$\sigma=50$} & DIP-TV & 
    $21.30\pm0.02$ & $24.00\pm0.10$ & $25.60\pm0.02$ & $25.29\pm0.08$ & $22.39\pm0.06$ & $25.14\pm0.02$ & $24.39\pm0.03$ \\
    & Ours &
    $21.05\pm0.05$ & $24.05\pm0.06$ & $25.79\pm0.06$ & $25.38\pm0.14$ & $22.33\pm0.08$ & $25.13\pm0.07$ & $24.33\pm0.07$ \\
    \midrule
    \multirow{2}{*}{$\sigma=75$} & DIP-TV & 
    $19.60\pm0.04$ & $22.28\pm0.01$ & $23.40\pm0.12$ & $23.18\pm0.02$ & $20.25\pm0.08$ & $22.13\pm0.06$ & $21.68\pm0.02$ \\
    & Ours &
    $19.55\pm0.03$ & $22.33\pm0.01$ & $23.53\pm0.02$ & $23.32\pm0.24$ & $20.13\pm0.07$ & $22.08\pm0.02$ & $21.72\pm0.08$ \\
    \midrule
    \multirow{2}{*}{$\sigma=100$} & DIP-TV & 
    $18.35\pm0.04$ & $20.62\pm0.06$ & $21.86\pm0.14$ & $21.56\pm0.14$ & $18.04\pm0.08$ & $19.68\pm0.02$ & $19.55\pm0.05$ \\
    & Ours &
    $18.39\pm0.05$ & $20.76\pm0.06$ & $21.88\pm0.05$ & $21.61\pm0.12$ & $18.56\pm0.05$ & $19.75\pm0.08$ & $19.60\pm0.02$ \\
    \bottomrule

    \toprule
    \multirow{2}{*}{\textbf{Noise Level}} & 
    \multirow{2}{*}{\textbf{Method}} & 
    \multicolumn{7}{c}{\textbf{Images}} \\
     & & \emph{8} & \emph{9} & \emph{10} & \emph{11} & \emph{12} & \emph{13} & \emph{14}  \\
    \midrule
    \multirow{2}{*}{$\sigma=25$} & DIP-TV & 
    $31.29\pm0.12$ & $30.40\pm0.08$ & $25.60\pm0.08$ & $29.00\pm0.01$ & $30.05\pm0.01$ & $27.96\pm0.03$ & $27.87\pm0.06$ \\
    & Ours &
    $31.21\pm0.11$ & $31.32\pm0.05$ & $25.47\pm0.09$ & $29.32\pm0.06$ & $29.99\pm0.05$ & $28.34\pm0.14$ & $27.71\pm0.06$ \\
    \midrule
    \multirow{2}{*}{$\sigma=50$} & DIP-TV & 
    $26.94\pm0.16$ & $27.60\pm0.02$ & $23.46\pm0.02$ & $25.42\pm0.03$ & $26.86\pm0.08$ & $23.02\pm0.03$ & $24.69\pm0.02$ \\
    & Ours &
    $27.00\pm0.05$ & $27.53\pm0.01$ & $23.32\pm0.04$ & $25.55\pm0.04$ & $26.85\pm0.03$ & $23.16\pm0.03$ & $24.81\pm0.01$ \\
    \midrule
    \multirow{2}{*}{$\sigma=75$} & DIP-TV & 
    $23.36\pm0.02$ & $24.73\pm0.02$ & $21.32\pm0.09$ & $22.52\pm0.06$ & $23.67\pm0.01$ & $19.69\pm0.10$ & $22.44\pm0.03$ \\
    & Ours &
    $23.52\pm0.04$ & $24.77\pm0.02$ & $21.25\pm0.05$ & $22.73\pm0.10$ & $23.86\pm0.05$ & $19.79\pm0.02$ & $22.52\pm0.03$ \\
    \midrule
    \multirow{2}{*}{$\sigma=100$} & DIP-TV & 
    $20.71\pm0.06$ & $22.38\pm0.06$ & $19.53\pm0.03$ & $20.02\pm0.01$ & $21.31\pm0.05$ & $17.22\pm0.05$ & $20.60\pm0.05$ \\
    & Ours &
    $20.87\pm0.04$ & $22.38\pm0.03$ & $19.59\pm0.02$ & $20.39\pm0.03$ & $21.34\pm0.02$ & $17.37\pm0.05$ & $20.64\pm0.04$ \\
    \bottomrule
\end{tabular*}
\end{center}
\caption{\textbf{Detailed image denoising quantitative results.}}
\label{ta:denoising_full}
\end{table*}



==> tables/l1vsUnrolled.tex <==
\begin{table}
\begin{center}
\begin{tabular}{l c c c c c} 
    \toprule
    %\textbf{Method} & \textbf{\underline{Sintel Clean}} & \textbf{\underline{Sintel Final}} \\
    \multirow{2}{4em}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{\underline{MPI Sintel}}} & \multicolumn{3}{c}{\textbf{\underline{KITTI 2015}}} \\
    & \emph{Clean} & \emph{Final} & \emph{Occ.} & \emph{Noc.} & \emph{All} \\
    \midrule
    Standard TV             & 2.47 & 3.47 & 6.51 & 2.16 & 2.91\\
    \textbf{Unrolled Cost}  & \textbf{2.35} & \textbf{3.19} & \textbf{5.48} & \textbf{2.14} & \textbf{2.82}\\
    \bottomrule
\end{tabular}
\end{center}
\caption{\textbf{TV norm vs. unrolled cost - validation.} 
    Studying the measured AEPE in occluded regions (\emph{Occ.}) demonstrates the effectiveness of our method even further, decreasing error rate by 15.82\%.
%We train our flow estimator using both an $L^1$ smoothness constraint and our proposed unrolled cost, on both the train sub-split of the MPI Sintel training data (see section \ref{ablations}) and the KITTI 2015 multi-view extension data, as explained in section \ref{datasets}, and report the AEPE. Our method achieves improved results in both cases, reducing EPE averaged on occluded regions by 15.82\% on the KITTI 2015 data.}
%We find our method particularly effective on motion boundaries, as AEPE measured on KITTI 2015 occluded regions (\emph{Occ.}) is reduced by 0.47px.}
}
\label{ta:l1vsunrolled}
\end{table}

==> tables/l1vsUnrolled_pwc.tex <==
\begin{table*}
\begin{center}
\begin{tabular*}{.9\linewidth}{@{\extracolsep{\fill}}l | c c c | c c c | c c c}
    \toprule
    %\textbf{Method} & \textbf{\underline{Sintel Clean}} & \textbf{\underline{Sintel Final}} \\
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{\underline{Sintel Clean}}} & \multicolumn{3}{c}{\textbf{\underline{Sintel Final}}} & \multicolumn{3}{c}{\textbf{\underline{KITTI 2015}}} \\
    & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} \\
    \midrule
    Standard TV                                     & 8.77 & 1.27 & 2.29 & 9.97 & 2.19 & 3.22 & 6.51 & 2.16 & 2.91\\
    Charbonnier \cite{charbonnier1997deterministic} & 8.96 & 1.31 & 2.34 & 9.98 & 2.20 & 3.22 & 6.23 & 2.13 & 2.89\\
    Huber \cite{huber1964robust}                    & 8.80 & 1.26 & 2.27 & 10.10 & 2.22 & 3.27 & 6.60 & 2.11 & 2.93 \\
    \textbf{Unrolled Cost (Ours)}  & \textbf{7.91} & 1.28 & \textbf{2.17} & \textbf{9.16} & 2.13 & \textbf{3.06} & \textbf{5.48} & 2.14 & \textbf{2.82}\\
    \bottomrule
\end{tabular*}
\end{center}
\caption{\textbf{Unrolled cost vs. TV relaxations - unsupervised optical flow.} Our method outperforms all tested $L^1$ relaxation baselines. Furthermore, our method decreases the TV EPE averaged over the occluded regions, which are highly affected by the smoothness constraint, by up to 15.82\%, enabling the detection of sharper motion boundaries without any modification to the model architecture or complexity.
%We train our flow estimator using both an $L^1$ smoothness constraint and our proposed unrolled cost, on both the train sub-split of the MPI Sintel training data (see section \ref{ablations}) and the KITTI 2015 multi-view extension data, as explained in section \ref{datasets}, and report the AEPE. Our method achieves improved results in both cases, reducing EPE averaged on occluded regions by 15.82\% on the KITTI 2015 data.}
%We find our method particularly effective on motion boundaries, as AEPE measured on KITTI 2015 occluded regions (\emph{Occ.}) is reduced by 0.47px.}
}
\label{ta:l1vsunrolled}
\end{table*}

==> tables/l1vsUnrolled_smurf.tex <==
\begin{table*}
\begin{center}
\begin{tabular*}{.9\linewidth}{@{\extracolsep{\fill}}l | c c c | c c c | c c c}
    \toprule
    %\textbf{Method} & \textbf{\underline{Sintel Clean}} & \textbf{\underline{Sintel Final}} \\
    \multirow{2}{*}{\textbf{RAFT Baseline}} & \multicolumn{3}{c}{\textbf{\underline{Sintel Clean}}} & \multicolumn{3}{c}{\textbf{\underline{Sintel Final}}} & \multicolumn{3}{c}{\textbf{\underline{KITTI 2015}}} \\
    & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} & \textbf{\emph{Occ.}} & \emph{Noc.} & \textbf{\emph{All}} \\
    \midrule
    Standard TV                                     & 8.88 & 1.10 & 2.17 & 10.46 & 2.08 & 3.25 & 6.43 & 2.31 & 3.17\\
    Charbonnier \cite{charbonnier1997deterministic} & 8.89 & 1.09 & 2.17 & 10.48 & 2.04 & 3.23 & 6.63 & 2.40 & 3.2\\
    Huber \cite{huber1964robust}                    & 8.68 & 1.07 & 2.11 & 10.56 & 2.08 & 3.27 & 6.96 & 2.21 & 3.13 \\
    \textbf{Unrolled Cost (Ours)}  & \textbf{8.24} & 1.10 & \textbf{2.07} & \textbf{9.88} & 2.11 & \textbf{3.16} & \textbf{6.14} & 2.30 & \textbf{3.09}\\
    \bottomrule
\end{tabular*}
\end{center}
\caption{\color{red} \textbf{Unrolled cost vs. TV relaxations - unsupervised optical flow.} Our method outperforms all tested $L^1$ relaxation baselines. Furthermore, our method decreases the TV EPE averaged over the occluded regions, which are highly affected by the smoothness constraint, by up to 15.82\%, enabling the detection of sharper motion boundaries without any modification to the model architecture or complexity.
%We train our flow estimator using both an $L^1$ smoothness constraint and our proposed unrolled cost, on both the train sub-split of the MPI Sintel training data (see section \ref{ablations}) and the KITTI 2015 multi-view extension data, as explained in section \ref{datasets}, and report the AEPE. Our method achieves improved results in both cases, reducing EPE averaged on occluded regions by 15.82\% on the KITTI 2015 data.}
%We find our method particularly effective on motion boundaries, as AEPE measured on KITTI 2015 occluded regions (\emph{Occ.}) is reduced by 0.47px.}
}
\label{ta:raft_results}
\end{table*}

==> tables/toy_admm.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{l c c} 
    \toprule
    \textbf{Unrolled Cost (ours)} & \textbf{Final Grad Norm} & \textbf{Pred. Error} \\
    \midrule
    %$\rho=0.001,\lambda=1.0$    & $7.88 \pm 0.87 \times10^{-10}$     & $1.76 \pm 0.60 \times10^{-2}$\\
    %$\rho=0.001,\lambda=0.1$    & $7.88 \pm 0.87 \times10^{-10}$     & $1.76 \pm 0.60 \times10^{-2}$\\
    $\rho=0.001,\lambda=0.00001$   & $1.05 \pm 0.30 \times10^{-9}$     & $1.76 \pm 0.71 \times10^{-2}$\\ 
    $\mathbf{\boldsymbol{\rho}=0.001,\boldsymbol{\lambda}=0.0001}$  & $\mathbf{7.82 \pm 0.79 \times10^{-10}}$     & $\mathbf{1.40 \pm 0.03 \times10^{-2}}$\\
    $\rho=0.001,\lambda=0.001$   & $2.53 \pm 2.53 \times10^{-9}$     & $1.75 \pm 0.62 \times10^{-2}$\\ 
    $\rho=0.001,\lambda=0.002$   & $3.35 \pm 3.63 \times10^{-9}$     & $2.11 \pm 0.74 \times10^{-2}$\\ 
    %$\rho=0.0005,\lambda=0.0005$ & $4.20 \pm 0.09 \times10^{-5}$     & $1.92 \pm 0.61 \times10^{-2}$\\
    %$\rho=0.01,\lambda=0.0005$ & $1.43 \pm 0.78 \times10^{-9}$      & $1.84 \pm 0.68 \times10^{-2}$\\ 
    %$\epsilon=1$        & $1.20 \pm 0.71 \times10^{-8}$     & $1.67 \pm 0.64\times10^{-2}$\\
    \bottomrule
\end{tabular}
\end{center}
\caption{\textbf{PC signal prediction - Unrolled cost ablations.}}
\label{ta:toy_admm}
\end{table}

==> tables/toy_charb.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{l c c} 
    \toprule
    \textbf{Charbonnier} & \textbf{Final Grad Norm} & \textbf{Pred. Error} \\
    \midrule
    $\epsilon=0.001$    & $3.83 \pm 0.02 \times10^{-5}$     & $2.25 \pm 0.79\times10^{-2}$\\
    $\epsilon=0.01$     & $3.37 \pm 0.05 \times10^{-5}$     & $2.19 \pm 0.77\times10^{-2}$\\
    $\epsilon=0.1$      & $4.36 \pm 0.37 \times10^{-9}$     & $2.04 \pm 0.69 \times10^{-2}$\\    
    $\mathbf{\boldsymbol{\epsilon}=1}$      & $\mathbf{1.2 \pm 0.71 \times10^{-8}}$     & $\mathbf{1.67 \pm 0.64 \times10^{-2}}$\\    
    $\epsilon=2$      & $1.15 \pm 0.65 \times10^{-8}$     & $1.81 \pm 0.83 \times10^{-2}$\\    

    %$\epsilon=1$        & $1.20 \pm 0.71 \times10^{-8}$     & $1.67 \pm 0.64\times10^{-2}$\\
    \bottomrule
\end{tabular}
\end{center}
\caption{\textbf{PC signal prediction - Charbonnier ablations.}}
\label{ta:toy_charb}
\end{table}

==> tables/toy_huber.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{l c c} 
    \toprule
    \textbf{Huber} & \textbf{Final Grad Norm} & \textbf{Pred. Error} \\
    \midrule
    $k=0.01$    & $1.55 \pm 0.10 \times10^{-7}$     & $3.07 \pm 0.42\times10^{-1}$\\
    $k=0.1$     & $2.69 \pm 0.14 \times10^{-7}$     & $1.65 \pm 0.30\times10^{-1}$\\
    $k=1$       & $6.72 \pm 5.28 \times10^{-9}$     & $1.91 \pm 0.73 \times10^{-2}$\\    
    $\mathbf{k=2}$       & $\mathbf{3.77 \pm 2.81 \times10^{-9}}$     & $\mathbf{1.62 \pm 0.65 \times10^{-2}}$\\    
    $k=4$       & $3.28 \pm 2.18 \times10^{-9}$     & $1.65 \pm 0.63 \times10^{-2}$\\    
    %$k=2$       & $3.77 \pm 2.81 \times10^{-9}$     & $1.62 \pm 0.64\times10^{-2}$\\
    \bottomrule
\end{tabular}
\end{center}
\caption{\textbf{PC signal prediction - Huber ablations.}}
\label{ta:toy_huber}
\end{table}
